Directly Determined Linear Radii and Effective Temperatures of Exoplanet Host Stars

We present interferometric angular sizes for 12 stars with known planetary companions, for comparison with 28 additional main-sequence stars not known to host planets. For all objects we estimate bolometric fluxes and reddenings through spectral energy distribution fits, and in conjunction with the angular sizes, measurements of effective temperature. The angular sizes of these stars are sufficiently small that the fundamental resolution limits of our primary instrument, the Palomar Testbed Interferometer, are investigated at the sub-milliarcsecond level and empirically established based upon known performance limits. We demonstrate that the effective temperature scale as a function of dereddened $(V-K)_0$ color is statistically identical for stars with and without planets. A useful byproduct of this investigation is a direct calibration of the $T_{\rm EFF}$ scale for solar-like stars, as a function of both spectral type and $(V-K)_0$ color, with an precision of $\bar{\Delta T}_{\rm {(V-K)}_0} = 138$K over the range $(V-K)_0=0.0-4.0$ and $\bar{\Delta T}_{\rm {SpType}} = 105$K for the range F6V -- G5V. Additionally, we provide in an appendix spectral energy distribution fits for the 166 stars with known planets which have sufficient photometry available in the literature for such fits; this derived "{\tt XO-Rad}" database includes homogenous estimates of bolometric flux, reddening, and angular size.

==> tab_starResults_LCV.tex <==
%\clearpage
%\begin{landscape}
\begin{deluxetable}{cccccc}
\tablecolumns{6}
\tablewidth{0pc}
\tablecaption{Unreddened colors, effective temperatures and radii for luminosity class V stars.\label{tableResults_LC5stars}}
\tablehead{
\colhead{Star ID} &
\colhead{$V_0-K_0$} &
\colhead{$T_{\rm EFF}$} &
\colhead{$d$} &
\colhead{$R$} \\
 &
\colhead{(mag)} &
\colhead{(K)} &
\colhead{(pc)} &
\colhead{$(R_\odot)$}
}
\tabletypesize{\scriptsize}
\startdata
\hline
\multicolumn{5}{l}{Control Sample: Stars not known to host planets:}\\
\hline
HD1326 & $4.095 \pm 0.053$ & $3584 \pm 105$ & $3.568 \pm 0.013 $ & $0.393 \pm 0.023 $ \\
HD4628 & $2.125 \pm 0.052$ & $4929 \pm 169$ & $7.460 \pm 0.048 $ & $0.749 \pm 0.051 $ \\
HD16160 & $2.247 \pm 0.052$ & $5262 \pm 216$ & $7.209 \pm 0.054 $ & $0.650 \pm 0.053 $ \\
HD16895 & $1.327 \pm 0.091$ & $6200 \pm 163$ & $11.232 \pm 0.100 $ & $1.313 \pm 0.069 $ \\
HD19373 & $1.395 \pm 0.071$ & $5722 \pm 110$ & $10.534 \pm 0.074 $ & $1.509 \pm 0.058 $ \\
HD20630 & $1.511 \pm 0.052$ & $5908 \pm 232$ & $9.159 \pm 0.065 $ & $0.882 \pm 0.069 $ \\
HD22484 & $1.358 \pm 0.101$ & $6618 \pm 449$ & $13.719 \pm 0.147 $ & $1.345 \pm 0.183 $ \\
HD30652 & $0.925 \pm 0.061$ & $7067 \pm 124$ & $8.026 \pm 0.061 $ & $1.217 \pm 0.043 $ \\
HD39587 & $1.404 \pm 0.071$ & $5766 \pm 144$ & $8.663 \pm 0.081 $ & $1.047 \pm 0.053 $ \\
HD87901 & $-0.352 \pm 0.061$ & $14231 \pm 314$ & $23.759 \pm 0.446 $ & $3.092 \pm 0.147 $ \\
HD88230 & $3.347 \pm 0.051$ & $4156 \pm 89$ & $4.873 \pm 0.019 $ & $0.649 \pm 0.028 $ \\
HD95735 & $4.031 \pm 0.051$ & $3593 \pm 60$ & $2.548 \pm 0.006 $ & $0.395 \pm 0.013 $ \\
HD97603 & $0.106 \pm 0.062$ & $8899 \pm 201$ & $17.693 \pm 0.260 $ & $2.281 \pm 0.106 $ \\
HD102647 & $0.194 \pm 0.052$ & $8759 \pm 158$ & $11.091 \pm 0.109 $ & $1.657 \pm 0.060 $ \\
HD109358 & $1.530 \pm 0.072$ & $5896 \pm 145$ & $8.371 \pm 0.058 $ & $1.025 \pm 0.050 $ \\
HD114710 & $1.311 \pm 0.100$ & $6167 \pm 165$ & $9.155 \pm 0.060 $ & $1.056 \pm 0.057 $ \\
HD119850 & $4.060 \pm 0.052$ & $3664 \pm 153$ & $5.431 \pm 0.037 $ & $0.481 \pm 0.040 $ \\
HD126660 & $1.175 \pm 0.073$ & $6358 \pm 161$ & $14.571 \pm 0.119 $ & $1.772 \pm 0.087 $ \\
HD141004 & $1.423 \pm 0.081$ & $6662 \pm 477$ & $11.754 \pm 0.111 $ & $1.060 \pm 0.152 $ \\
HD142860 & $1.168 \pm 0.062$ & $6496 \pm 153$ & $11.121 \pm 0.089 $ & $1.389 \pm 0.065 $ \\
HD149661 & $1.648 \pm 0.052$ & $5196 \pm 196$ & $9.778 \pm 0.081 $ & $0.934 \pm 0.070 $ \\
HD157881 & $3.419 \pm 0.052$ & $4030 \pm 242$ & $7.720 \pm 0.057 $ & $0.564 \pm 0.068 $ \\
HD185144 & $1.845 \pm 0.081$ & $5628 \pm 148$ & $5.767 \pm 0.015 $ & $0.678 \pm 0.035 $ \\
HD201091 & $2.546 \pm 0.051$ & $4526 \pm 66$ & $3.482 \pm 0.018 $ & $0.610 \pm 0.018 $ \\
HD201092 & $3.431 \pm 0.051$ & $4077 \pm 59$ & $3.503 \pm 0.009 $ & $0.628 \pm 0.017 $ \\
HD210027 & $1.267 \pm 0.071$ & $6359 \pm 141$ & $11.756 \pm 0.098 $ & $1.526 \pm 0.068 $ \\
HD215648 & $1.243 \pm 0.082$ & $6461 \pm 190$ & $16.250 \pm 0.203 $ & $1.787 \pm 0.106 $ \\
HD222368 & $1.245 \pm 0.081$ & $6521 \pm 179$ & $13.791 \pm 0.167 $ & $1.577 \pm 0.087 $ \\
\hline
\multicolumn{5}{l}{EHSA Sample: Known planet hosting stars (PTI):}\\
\hline
HD3651 & $1.847 \pm 0.052$ & $5457 \pm 325$ & $11.107 \pm 0.089 $ & $0.818 \pm 0.098 $ \\
HD9826 & $1.239 \pm 0.081$ & $6465 \pm 188$ & $13.468 \pm 0.131 $ & $1.480 \pm 0.087 $ \\
HD28305 & $2.168 \pm 0.052$ & $4990 \pm 50$ & $47.529 \pm 1.852 $ & $12.692 \pm 0.545 $ \\
HD75732 & $1.935 \pm 0.221$ & $4952 \pm 216$ & $12.531 \pm 0.132 $ & $1.100 \pm 0.096 $ \\
HD95128 & $1.180 \pm 0.341$ & $6140 \pm 294$ & $14.077 \pm 0.131 $ & $1.172 \pm 0.111 $ \\
HD117176 & $1.625 \pm 0.052$ & $5687 \pm 188$ & $18.109 \pm 0.239 $ & $1.858 \pm 0.124 $ \\
HD120136 & $0.933 \pm 0.053$ & $6680 \pm 260$ & $15.596 \pm 0.170 $ & $1.450 \pm 0.112 $ \\
HD143761 & $1.439 \pm 0.052$ & $5936 \pm 339$ & $17.428 \pm 0.216 $ & $1.306 \pm 0.149 $ \\
HD217014 & $1.432 \pm 0.051$ & $5800 \pm 338$ & $15.361 \pm 0.179 $ & $1.141 \pm 0.133 $ \\
\hline
\multicolumn{5}{l}{EHSA Sample: Known planet hosting stars (CHARA):}\\
\hline
HD3651 & $1.885 \pm 0.038$ & $5059 \pm 87$ & $11.107 \pm 0.089 $ & $0.818 \pm 0.098 $ \\
HD11964 & $1.543 \pm 0.022$ & $5417 \pm 354$ & $0.000 \pm 0.000 $ & $2.234 \pm 0.304 $ \\
HD19994 & $1.189 \pm 0.238$ & $6109 \pm 112$ & $0.000 \pm 0.000 $ & $1.898 \pm 0.070 $ \\
HD75732 & $1.831 \pm 0.042$ & $4835 \pm 77$ & $12.531 \pm 0.132 $ & $1.100 \pm 0.096 $ \\
HD143761 & $1.469 \pm 0.039$ & $5981 \pm 194$ & $17.428 \pm 0.216 $ & $1.306 \pm 0.149 $ \\
HD189733 & $2.051 \pm 0.028$ & $4953 \pm 163$ & $0.000 \pm 0.000 $ & $0.781 \pm 0.051 $ \\
HD217014 & $1.511 \pm 0.023$ & $5570 \pm 100$ & $15.361 \pm 0.179 $ & $1.141 \pm 0.133 $ \\
\enddata
\end{deluxetable}
%\clearpage
%\end{landscape}


==> tab_teff_sptype.tex <==
%\clearpage
%\begin{landscape}
\begin{deluxetable}{cccc}
\tablecolumns{4}
\tablewidth{0pc}
\tablecaption{Effective temperature versus spectral type.\label{table_teff_sptype}}
\tablehead{
\colhead{Spectral} &
\colhead{$N$} &
\colhead{$T_{\rm EFF}$} &
\colhead{$T_{\rm EFF, Cox}$} \\
\colhead{Type} &
\colhead{} &
\colhead{(K)} &
\colhead{(K)}
}
\tabletypesize{\scriptsize}
\startdata
F6V & 6 & $6582 \pm 64$ & 6517 \\
F8V & 4 & $6206 \pm 81$ & 6250 \\
G0V & 7 & $5844 \pm 66$ & 5940 \\
G2V & 2 & $5590 \pm 97$ & 5790 \\
G5V & 4 & $5507 \pm 115$ & 5560 \\
K1V & 4 & $4966 \pm 53$ & 4990 \\
K7V & 3 & $4099 \pm 48$ & 4125 \\
M2V & 3 & $3599 \pm 49$ & 3520\\
\enddata
\tablecomments{See discussion at end of \S \ref{sec_temperatures}. $N$ is the number of angular size measurements per spectral type; columns 3 and 4 are from this work and \citet{cox00}, respectively.}
\end{deluxetable}
%\clearpage
%\end{landscape}
%\clearpage

